Regret Bounds and Regimes of Optimality for User-User and Item-Item Collaborative Filtering

We consider an online model for recommendation systems, with each user being recommended an item at each time-step and providing 'like' or 'dislike' feedback. Each user may be recommended a given item at most once. A latent variable model specifies the user preferences: both users and items are clustered into types. All users of a given type have identical preferences for the items, and similarly, items of a given type are either all liked or all disliked by a given user. We assume that the matrix encoding the preferences of each user type for each item type is randomly generated; in this way, the model captures structure in both the item and user spaces, the amount of structure depending on the number of each of the types. The measure of performance of the recommendation system is the expected number of disliked recommendations per user, defined as expected regret. We propose two algorithms inspired by user-user and item-item collaborative filtering (CF), modified to explicitly make exploratory recommendations, and prove performance guarantees in terms of their expected regret. For two regimes of model parameters, with structure only in item space or only in user space, we prove information-theoretic lower bounds on regret that match our upper bounds up to logarithmic factors. Our analysis elucidates system operating regimes in which existing CF algorithms are nearly optimal.

==> ItemUpper.tex <==
\section{Item-item algorithm and analysis}
\label{s:itemitem}

This section describes a version of item-item CF with explicit exploration steps and analyzes its performance within the setup described in Section~\ref{sec:model}. 



\subsection{Algorithm}\label{ss:itemalg}
Algorithm \textsc{Item-Item} performs the following steps (see Algorithm~\ref{alg:item-fixed}). First, items are partitioned according to type; next, each user's preference for each item type is determined; finally, items from liked partitions are recommended. These steps are now described in a bit more detail. 

Two sets $\Mcc$ and $\Mcct$, each containing $M$ random items, are selected. In the exploration step, each item is recommended to $\thr=\lceil 2\log(\qi/\epsilon)\rceil$ random users. The feedback from these recommendations later helps to partition the items according to type. The parameter $\thr$ is chosen large enough to guarantee small probability of error in partitioning ($\leq \epsilon$ for each item). The use of two sets $\Mcc$ and $\Mcct$, as opposed to just one, is to simplify the analysis; as described next, item type representatives are selected from $\Mcct$, and are used to represent clusters of items from $\Mcc$. 

An item from each of $\ell$ \emph{explored types} is recommended to all users, where $\ell$ is a parameter determined by the algorithm.
It turns out that it is often beneficial (depending on system parameters) to learn user preferences for only a subset of the types, in which case $\ell$ is strictly less than $\qi$.  Each of the $\ell$ items chosen from $\Mcct$ is thought of as a \emph{representative} of its type. 
For each $j=1,\dots,\ell$, all items in $\Mcct$ that appear to be of the same type as the representative item $\rep_{\ti}$ are stored in a set $\St{2}_\ti$ and then removed from $\Mcct$. This guarantees that at each time $\Mcct$ does not contain items with the same type as any of the previously selected representative items. 
For each $j=1,\dots,\ell$, all items in $\Mcc$ that appear to be of the same type as  $\rep_{\ti}$ are stored in a set $\St{1}_\ti$ and then removed from $\Mcc$. 

For each user $u$, we add the items in the groups $\St{1}_\ti$ whose representative $\rep_\ti$ were liked by $u$ to the set of exploitable items $\R_u\,$ by $u$.
Finally, in the exploitation phase, each user is recommended items from $\R_u$.
We choose the number $M$ of items in each of $\Mcc$ and $\Mcct$  as a function of $\ell$ to ensure that there are enough exploitable items in $\R_u$ for all users $u$ for the entire length-$T$ time-horizon. Then, $\ell$ is chosen to minimize regret.

The algorithm description uses the following notation. 
For an item $i$ and time $t>0$, $$\rated_t(i) = \{u\in [N]: a_{u,s}= i \text{ for some } s<t\}$$ is the set of users that have rated item $i$ before time $t$. 
The time $t$ is implicit in the algorithm description, with $\rated(i)$ used to represent $\rated_t(i)$ at the time of its appearance.

\begin{theorem}\label{th:Item-upper} Suppose that $\qi,\qu>18\log(3N)$. 
	Let $\thr=\lceil 2\log(2N\qi^2) \rceil$. Then \textsc{Item-Item} (Algorithm \ref{alg:item-fixed}) obtains regret per user at time $T$ upper bounded as 
\[\reg(T)\leq 4+ 57 \max\left\{\log T \, ,\, \sqrt{3\frac{\qi \thr}{N}T} ,\, 53 \frac{\thr}{N} T\right\}\,.\]
\end{theorem}
The simplified version of this theorem in Section \ref{s:results} is otained using $N\geq \qu$, which gives $2\log N< \thr<7\log N$ and $N>3$.\MK{double check the statement and the assumptions of the theorem. }

\begin{algorithm}
\caption{$\textsc{Item-Item}(T, \qi, N)$ (fixed time horizon)}\label{alg:item-fixed}
\begin{algorithmic}[1]

\State $\ell =\min\Big\{\left\lceil 18\log T+ \sqrt{330\frac{\qi \thr}{ N}T}\,\,\right\rceil,\qi\Big\}$	\vspace{1mm}

		\vspace{1mm}
\State $\epsilon= \frac{1}{2 \qi N}$; $\thr = \left\lceil 2\log\frac{\qi}{\epsilon}\right\rceil$;  $M=\left\lceil \frac{64\qi}{\ell} T \right\rceil$
\vspace{.2cm}
\State $\Mcc \gets M$  random items; $\Mcct\gets M$  new random items
\vspace{.1cm}
		\vspace{1mm}
\State $\R_u\gets\varnothing, \text{ for each } u\in[N]$ \quad (items exploitable by user $u$)
\vspace{.2cm}
\State $ \{\R_u\}_{u\in [N]}\gets  \textsc{ItemExplore}(\Mcc, \Mcct, \ell)$
\vspace{.2cm}
\State $\textsc{ItemExploit}(\{\R_u\}_{u\in [N]})$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{$\textsc{ItemExplore}(\Mcc, \Mcct, \ell)$}\label{alg:itemExplore}
	\begin{algorithmic}[1]
	\State $\St{1}_\ti\gets\varnothing, \quad \ti\in[\qi]$ \quad (initialize sets of items of type $j$ in $\Mcc$)
	\State $\St{2}_\ti\gets\varnothing, \quad \ti\in[\qi]$ \quad (initialize sets of items of type $j$ in $\Mcct$)
	
\vspace{2mm}
		\Statex \emph{Rate items by a few users (preliminary exploration)}
\State Recommend each item in $\Mcc$ and $\Mcct$ to $\thr$ users from $[N]$ (details specified in Remark~\ref{r:usersToItems}).  \label{line:ItemExplore-initialallocation}
		\vspace{2mm}
		\Statex \emph{Partition items and learn item types} 
		\For{$\ti=1,\cdots,\ell$ \textbf{if} $\Mcct\neq \varnothing$} 
		\State $\rep_\ti \gets$ a random item in $\Mcct$ (a representative item)
		\State $a_{u,t}\gets \rep_\ti$ if $u\notin\rated(\rep_{\ti})$, otherwise a random item not from $\Mcct$ \MK{why shouldn't it be from $\Mcct$}
%		\State Let $U_{i,\rep_\ti} = \rated(i)\cap \rated(\rep_{\ti})$ for each $i$ and $\rep_\ti$
		\State $\St{1}_\ti \gets \big\{i\in \Mcc: L_{u, i} = L_{u,\rep_\ti}\text{ for all } u\in \rated(i)\cap \rated(\rep_{\ti})\big\}$,  \quad (users agree on $i$ vs. $\rep_\ti$)
		\vspace{.07cm}
		\State $\Mcc\gets \Mcc\setminus \St{1}_\ti$ 
 		\vspace{.07cm}
			\State $\St{2}_\ti \gets \big\{i\in \Mcct: L_{u, i} = L_{u,\rep_\ti} \text{ for all } u\in \rated(i)\cap \rated(\rep_{\ti})\big\}$
			 		\vspace{.07cm}
		\State $\Mcct\gets \Mcct\setminus \St{2}_\ti $
		\EndFor  
		\State $\R_u = \bigcup_{j\in[\ell]:L_{u,\rep_\ti}=+1} \St{1}_j\,\,\,$ for each $u\in [N]$
		\label{Line-alg:ItemUpperRu}
	\end{algorithmic} 
\Return  $\{\R_u\}_{u\in [N]}$
\end{algorithm}

\begin{algorithm}
	\caption{$\textsc{ItemExploit}(\{\R_u\}_{u\in [N]})$}\label{alg:itemExploit}
	\begin{algorithmic}[1]
\For{ remaining $ t \leq T $}
\For{$u\in [N]$}
\If{there is an item $i \in\R_u$ such that $u\notin \rated_t(i)$,} 
\State $a_{u,t}\gets i$ 
\Else  { } $a_{u,t} \gets$ a random item not yet rated by $u$.
\EndIf
\EndFor
\EndFor
	\end{algorithmic}
\end{algorithm}


\begin{remark} 
The set of items $\Mcc$ and $\Mcct$ are updated throughout the algorithm $\textsc{ItemExplore}$. 
In the proof,  we use the notation 
$\Mcc_0$ and $\Mcct_0$ to refer to the set of items $\Mcc$ and $\Mcct$ at the beginning of the algorithm $\textsc{Item-Item}$. 
\end{remark}
\begin{remark} \label{r:usersToItems}
Assignment of users to items for Line~\ref{line:ItemExplore-initialallocation} of {\sc ItemExplore}: This is done over $\lceil{(|\Mcc_0|+|\Mcct_0|)\thr}/{N}\rceil\leq 2M\thr/N+1$ time-steps, with additional recommendations being random new items. The main requirement in assigning users to items is to make Claim~\ref{cl:Ftilde} below ( which bounds the probability of mis-classification of each item) hold.
 Since the claim addresses each item separately, we may introduce dependencies between sets of users for different items. What is important is that the set of users assigned to each specific item is uniform at random among all sets of users (or at least contains a random size $\thr$ subset). For example, one can choose a random permutation for the users, repeat this list $\lceil{(|\Mcc_0|+|\Mcct_0|)\thr}/{N}\rceil\leq 2M\thr/N+1$ times, and then assign each item to a block of $\thr$ users.
\end{remark}




\subsection{Proof of Theorem~\ref{th:Item-upper}}

We now prove Theorem~\ref{th:Item-upper}, deferring several lemmas and claims to Section~\ref{sec:ItemUpper-Lemmas}.


The basic error event is misclassification of an item. In  \textsc{ItemExplore} (Alg.~\ref{alg:itemExplore}), $\St{1}_\ti$ is the set of items in $\Mcc$ that the algorithm posits are of the same type as the $j$-th representative $\rep_\ti\,.$ 
 Let $\EE^1_i$ be the event that item $i$ was mis-classified, 
		\begin{equation}\label{e:EE}
		\EE^1_i = \{\exists \ti : i\in\St{1}_\ti, \tau_I(i)\neq \tau_I(\rep_\ti)\}\,.
		\end{equation}
		\MK{do I absolutely have to differentiate between $	\EE^1_i $ and $\EE^2_i $?  }
	The number of time-steps spent making recommendations in \textsc{ItemExplore} is denoted by $\Tu$.
We partition the recommendations made by Algorithm \textsc{Item-Item} to decompose the regret 
as follows:
\begin{align}
N\reg(T) & =  \Exp{ \sum_{u=1}^N\sum_{t=1}^{\Tu} \ident[L_{u,a_{u,t}}=-1]}\notag\\
&\quad + \Exp{ \sum_{u=1}^N\sum_{t=\Tu+1}^T  \ident[L_{u,a_{u,t}}=-1, a_{u,t}\notin\R_u]}\notag\\
& \quad +  \Exp{ \sum_{u=1}^N\sum_{t=\Tu +1}^T  \ident[L_{u,a_{u,t}}=-1, a_{u,t}\in\R_u, \EE^1_{a_{u,t}}]}\notag\\
& \quad +  \Exp{ \sum_{u=1}^N\sum_{t=\Tu+1}^T \ident[L_{u,a_{u,t}}=-1, a_{u,t}\in\R_u, (\EE^1_{a_{u,t}})^c]} \notag\\
& =: \Asf{1} + \Asf{2} + \Asf{3} + \Asf{4}\,. \label{eq:IU-reg-decomp}
\end{align}
The first term, $\Asf{1}$, is the regret from early time-steps up to $\Tu$. The second term,  $\Asf{2}$, is the regret due to not having enough items available for the exploitation phase, which is proved to be small with high probability for sufficiently large $M$. The third term, $\Asf{3}$, is the regret due to exploiting the misclassified items. It is small since few items are misclassified with the proper choice of $\epsilon$ and $\thr$. The fourth term, $\Asf{4}$, is the regret due to exploiting the correctly classified items. We will see that $\Asf{4}=0\,.$
\paragraph{Bounding $\Asf{1}$.}
 Line~\ref{line:ItemExplore-initialallocation} of \textsc{ItemExplore} takes at most $\big\lceil\frac{2M\thr}{N}\big\rceil$ units of time to rate each item in $\Mcc_0$ and $\Mcct_0$ by $\thr$ users each, since $N$ users provide feedback at each time-step. 
 Remark~\ref{r:usersToItems} discusses the assignment of users to items in this phase.
 After this, $\ell$ representative items are rated by every user in the for loop (lines 4 through 10 of \textsc{ItemExplore}),
 which takes $\ell$ time-steps. 
 This gives
\[\Tu \leq  \bigg\lceil\frac{2M\thr}{N}\bigg\rceil + \ell  \leq  \frac{2M\thr}{N} + \ell +1 \,.\] 
For $t\leq \Tu\,,$ from the perspective of any user the items recommended to it are of random type and hence 
\begin{align}
\Asf{1} & =  \Exp{\sum_{u=1}^N \sum_{t=1}^{\Tu} \ident[L_{u,a_{u,t}}=-1]} = \frac{1}{2}\sum_{u=1}^N \Tu \leq   {M\thr} + \frac{1}{2}(\ell +1)N \,.\label{eq:IU-bound-A}
\end{align}
\paragraph{Bounding $\Asf{2}$.}
Time-steps $t>\Tu$ are devoted to exploitation as described in \textsc{ItemExploit}. 
During this phase, a random item $a_{u,t}\notin \R_u$ is recommended to user $u$ only when there are no items to exploit because all items in $\R_u$ have already been recommended to $u$. So, the total number of times an item $a_{u,t}\notin \R_u$ is recommended in the time interval $\Tu <  t\leq T$ is at most $(T-|\R_u|)_+$, and
\begin{align}
\Asf{2} &= \Ex\bigg[{\sum_{u\in[N]} {\sum_{t=\Tu+1}^T \ident[L_{u,a_{u,t}}=-1, a_{u,t}\notin \R_u]}}\bigg] \leq
\Ex \bigg[{  \sum_{u\in [N]}  {\sum_{t=\Tu+1}^T \ident[ a_{u,t}\notin \R_u]}}\bigg]\notag\\
&\leq \sum_{u\in [N]} \Exp{(T -|\R_{u} |)_+} \leq 3TN\exp(-{\ell}/{18})+ 148T
\,,
 \label{eq:IU-bound-B}
\end{align}
where the last inequality is from Lemma~\ref{l:IU-exp-R-u} in Section~\ref{sec:ItemUpper-Lemmas}.

\paragraph{Bounding $\Asf{3}$.}
Term $\Asf{3}$ in~\eqref{eq:IU-reg-decomp} is the expected number of mistakes made by the Algorithm {\sc ItemExploit} as a result of misclassification. Claim~\ref{cl:iu-error-indep2} below upper bounds the expected number of ``potential misclassifications'' (defined in Equation~\eqref{eq:Ftilde}) in the algorithm to provide an upper bound for this {quantity}: 
\begin{align}
	\Asf{3}& = \Ex\bigg[{\sum_{u=1}^N \sum_{t=\Tu+1}^T  \ident[L_{u,a_{u,t}}=-1, a_{u,t}\in\R_u, \EE^1_{a_{u,t}}]}\bigg]
	\notag\\
	& \leq  \Ex\bigg[{\sum_{u=1}^N \sum_{t=\Tu+1}^T \sum_{i\in\mathbb{N}} \ident[a_{u,t}=i, i\in\R_u, \EE^1_i]} \bigg]\notag
	\\&
	\overset{\textrm{Claim}~\ref{cl:iu-error-indep2}}{\leq}  2 N M \epsilon \leq \frac{M}{\qi}\,.\label{eq:IU-bound-C}
\end{align}
%
\paragraph{Bounding $\Asf{4}$.}
By definition of the mis-classification  event, $\EE^1_i$, given in Equation~\eqref{e:EE}, if an item $i\in\St{1}_{\ti}\,$ is correctly  classified, then $\tau_I(i)=\tau_I(\rep_{\ti})$. 
User preferences for an item depend only on the type of the item (since $L_{u,i} = \xi_{\tau_U(u),\tau_I(i)}$), so all users rate $i$ the same as $\rep_{\ti}\,$. 
By construction of the sets $\R_u$ in Line~\ref{Line-alg:ItemUpperRu} of  {\sc ItemExploit}, for any item $i\in\R_u$, there is some $\ti\in[\qi]$ such that $i\in\St{1}_{\ti}$ and $u$ likes item $\rep_{\ti}\,$.
 Hence,
\begin{align}
\Pr[L_{u,i}=-1| i\in\R_u, (\EE^1_i)^c ] &= \Pr[L_{u,i}=-1| \exists \ti: L_{u,\rep_\ti}=+1, i\in\St{1}_{\ti}, \tau_I(i)= \tau_I(\rep_\ti)]\notag\\
& = \Pr[L_{u,i}=-1| \xi_{\tau_U(u),\tau_I(i)}=+1] =0\,.\label{eq:IU-bound-D}\notag
\end{align}
It follows that $\Asf{4} = 0$.
%
\MK{Double check from here on}
\paragraph{Combining all the bounds.}
Plugging in Equations~\eqref{eq:IU-bound-A},~\eqref{eq:IU-bound-B},~\eqref{eq:IU-bound-C} and~$\Asf{4} = 0$ into Equation~\eqref{eq:IU-reg-decomp} gives
\begin{align*}
N\reg(T) 
&\leq M\thr + \frac{1}{2} (\ell+1) N+3TN\exp\Big(-\frac{\ell}{18}\Big)+ 148T + \frac{M}{\qi}\,.
\end{align*}
Setting $M=\frac{64T\qi}{\ell}$ gives
\begin{align*}
\reg(T)
& \overset{(a)}{\leq} 
\frac 12 + 165  \frac{T\qi \thr}{\ell N} + \frac{\ell}{2}  + 3T\exp\Big(-\frac{\ell}{18}\Big)
\\
 &\overset{(b)}{\leq} 
\begin{cases}
5+ 18\log T+ \sqrt{330\frac{\qi \thr}{ N}T\,}\, &\text{ if } \ell<\qi\\
\frac{\qi}{2}+ 3T\exp\Big(-\frac \qi{18}\Big) + 330\frac{\thr}{N}T
&\text{ if } \ell = \qi
\end{cases}\\
&
\leq 
\begin{cases}
5+ 18\log T+ \sqrt{330\frac{\qi \thr}{ N}T\,}\, 
&\text{ if } T\leq \min\big\{\exp(\qi/36), \frac{N\qi}{660 \thr}\big\}\\
\frac{\qi}{2}+ 3T\exp\Big(-\frac \qi{18}\Big) + 330\frac{\thr}{N}T
&\text{otherwise}
\end{cases}
\end{align*}
%
%
where (a) holds for $\ell\geq 4$ (which is imposed by the algorithm) and
(b) is obtained by choosing the parameter $\ell$ to be $$\ell =\min\left\{\left\lceil 18\log T+ \sqrt{330\frac{\qi \thr}{ N}T}\,\,\right\rceil,\qi\right\}\,.$$ 
We can simplify the bound on regret by removing the term $3T\exp\Big(-\frac \qi{18}\Big)$: since $\qi>18\log(3N)$, the term can be absorbed into the last item in the max, yielding
%Note that $\thr=\log(N\qi^2)\leq 3\max\{\log N, \log \qi\}$. By assumption $\qi>18\log(3N),$ and for $N\geq 1$ it also holds that $\qi>18\log(3\qi)$. It follows that $3\exp(-\qi/18)<1/N$ and 
\begin{equation*}
\reg(T)
< 
\begin{cases}
\frac{T}{2}\quad &\text{ if } T<\max\big\{200, 1500 \frac{\qi \thr}{N}\big\}\\
4+ 57 \max\left\{\log T \, ,\, \sqrt{3\frac{\qi \thr}{N}T} ,\, 53 \frac{\thr}{N} T\right\}\quad &\text{otherwise}\,.
\end{cases}\qed
\end{equation*} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Lemmas used in the proof}\label{sec:ItemUpper-Lemmas}
In the remainder of this section we state and prove the lemmas used in the analysis above.
\begin{claim}\label{cl:iu-error-indep2}
Suppose that $\qu>4\thr$.
The expected total number of times a misclassified item is recommended in the exploitation step is upper bounded as
\[ \Exp{\sum_{u=1}^N \sum_{t=\Tu+1}^T \sum_{i\in\mathbb{N}} \ident[a_{u,t}=i, i\in\R_u, \EE^1_i]}\leq  N M  \epsilon\,.\]
\end{claim}
\begin{proof} 
Event $\EE^1_i$, defined in~\eqref{e:EE} to be the misclassification of item $i\in\Mcc$, occurs if the preferences of random users classifying item $i$ is the same as for a previous representative item with a different type. 
Given matrix $\Xi$, this event is a function of the order of choosing the representative items and the choice of random users in Line~\ref{line:ItemExplore-initialallocation} of {\sc ItemExplore}. 
Instead of directly analyzing $\EE^1_i$, we define an event called ``potential error event'' $\EEb_{i,U_i}$, which will be shown to satisfy $\EE^1_i\subseteq\EEb_{i,U_i}$; an upper bound for $\Pr[\EEb_{i,U_i}]$  is given in Claim~\ref{cl:Ftilde}.

For item $i$ and subset of users $U\subseteq [N]\,,$ define 
\begin{equation}
\label{eq:Ftilde}
\EEb_{i,U} =\{\exists \ti\neq \tau_I(i): L_{u,i}=\xi_{\tau_U(u),\ti}\,, \text{ for all } u\in U\}
\end{equation}
 to be the event that the ratings of users in $U$ for item $i$ agree with some other item type. 
For item $i\in\St{1}_{\ti}$, if $t$ is the time $i$ is added to $\St{1}_{\ti}$ in the exploration phase, let $U_i=\rated_t(i)\cap\rated_t(\rep_{\ti})$ be the set of witness users whose ratings were used to conclude that $i$ and $\rep_{\ti}$ are of the same type. 
Item $i$ is added to $\St{1}_{\ti}$ only if all users in $U_{i}$ agree on $i$ vs. $\rep_{\ti}\,$, so misclassification $\EE^1_i$ (defined in Equation~\eqref{e:EE}) implies $\EEb_{i,U_i}$. 
We can now deduce the inequalities, justified below:
\begin{align*}
\Ex \bigg[\sum_{u=1}^N \sum_{t=\Tu+1}^T \sum_{i\in\mathbb{N}} \ident[a_{u,t}=i, i\in\R_u, \EE^1_i]\bigg]
& \overset{(a)}{\leq}\Ex\bigg[{\sum_{u=1}^N \sum_{t=\Tu+1}^T\sum_{i\in\Mcc_0} \ident[a_{u,t}=i, i\in\R_u, \EEb_{i,U_i}]} \bigg]\\
%& \leq \Ex{\sum_{u=1}^N \sum_{t=\Tu{u}+1}^T \sum_{i\in\Mcc} \ident[a_{u,t}=i, \EEb_{i,U_i}]} \\
& \overset{(b)}{\leq}  N\Ex\bigg[{\sum_{i\in\Mcc} \ident[\EEb_{i,U_i}]}\bigg]\\
% \leq N M \max_{i\in\Mcc}\Pr[\EEb_{i,U_i}]\\
&\overset{(c)}{\leq} 2 N M  \epsilon\,.
\end{align*}%
 Inequality (a) holds because according to Line~\ref{Line-alg:ItemUpperRu} of {\sc ItemExplore} for every user $u\,$, the set $\R_u$ is a subset of $\Mcc_0$, and also the containment $\EE_i\subseteq \EEb_{i,U_i}$;
(b) follows since each item $i$ is recommended at most $N$ times; 
(c) uses $|\Mcc_0|= M$ together with Claim~\ref{cl:Ftilde} which shows that $\Pr[\EEb_{i,U_i}]\leq 2\epsilon$.
\end{proof}

\begin{claim}\label{cl:Ftilde} Suppose that $\qu>4\thr$.
Consider the ``potential error" event $\EEb_{i,U_i}$ defined in \eqref{eq:Ftilde} with the set of users $U_i$ defined immediately after. 
Then
$\Pr[\EEb_{i,U_i}] \leq 2\epsilon$ for all $i\in\Mcc_0$.
\end{claim}

\begin{proof}
 Each representative item $\rep_j$ chosen in $\textsc{ItemExplore}$ is rated by all of the users.
Other items in $\Mcc_0$ and $\Mcct_0$ are rated by at least $\thr$ users in the exploration phase. 
Remark~\ref{r:usersToItems} describes how Line~\ref{line:ItemExplore-initialallocation} in {\sc ItemExplore} is performed to guarantee that the set of $\thr$ users assigned to each specific item is uniformly at random among all subset of users of size $\thr$. 
By Lemma~\ref{l:ballsbins}, if $\qu>4\thr$, then with probability at least $1-\exp(-\thr/2)\geq 1-\epsilon/\qi$ there are $\thr/2$ users with distinct user types in a specific~$U_i$.
 It follows that the $\thr/2$ users with distinct types (chosen independently of the feedback) that rate item $i$ of type $\tau_{I}(i)$ also have the same ratings for type $j\neq \tau_{I}(i)$
 with probability at most $2^{-\thr/2}$. 
 (Any two item types $j\neq j'$ have jointly independent columns in the preference matrix.) The choice $\thr\geq 2\log({\qi}/{\epsilon})$ and a union bound over item types $\ti$ completes the proof. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{l:IU-exp-R-u}
For user $u\in[N],$ let $\R_{u}$ be defined as in Line 10 of algorithm \textsc{ItemExplore}. 
Then
\[\Pr\big[\,|\R_u|\leq T\,\big] \leq 3\, e^{-\nicefrac{\ell}{18}}\,+\,\tfrac{148}{N}\,,\]
and 
\[\Exp{(T- |\R_u |)_+} \,\leq\, 3\, T\, e^{-\nicefrac{\ell}{18}}+ \tfrac{148}{N}T\,.\]
\end{lemma}

\begin{proof}%[Proof of Lemma \ref{l:IU-exp-R-u}:]
We begin with a sketch. 
Any user $u$ likes roughly half of the  $\ell$ item types  that have representatives $\{\rep_j\}_{j=1}^\ell$. The total number of items in $\Mcc_0$ is $\tfrac{64\,\qi}{\ell}T$, so there are about $\frac{64}{\ell}T$ items from each of the item types in $\Mcc_0$. 
Adding over the $\ell$ types, the set $\R_u$ of items in $\Mcc_0$ that user $u$ likes will typically have size at least~$T$. 

Making this argument rigorous requires some care for the following reasons: 
1) $\R_u$ is the union of the $\St{1}_{\ti}$'s with $L_{u,\rep_{\ti}}=+1$, but $\St{1}_{\ti}$ can be missing items
due to misclassification (there may be items of the same type as  $\rep_{\ti}$ that have been classified as being of the same type as some $\rep_{j'}$ for which $L_{u,\rep_{\ti'}}=-1$).
2) The distribution of the type of each  representative item depends on the number of remaining items of each type in $\Mcc$ when the representative is chosen.  
Again, due to misclassification, this can be different from the actual number of items of each type initially present in $\Mcc$. Moreover, because misclassification of an item depends on the ratings of users for the item, the choice of next item type to be represented is therefore dependent on ratings of users for other types. 
The effect of this dependence is addressed in Claim~\ref{cl:IU-lukbd} below.

We now proceed with the proof, bounding the size of $\R_u$ by introducing a different set.
 For $u\in[N]$, let
\begin{equation}\label{eq:IU-Ruk}
\Rt^1_{u}=\{i\in\Mcc_0: \tau_I(i)=\tau_I(\rep_{\ti}), \text{ for some }\ti\in[\ell] \text{ such that } L_{u,\rep_{\ti}}= +1\}
\end{equation} 
be the items in $\Mcc_0$ whose types are the same as one of the representatives $\rep_{\ti}$ that are liked by $u$.
Note that if an item $i\in \Rt^1_{u}$ is correctly classified by the algorithm (i.e. $(\EE^1_i)^c$ occurs, where $\EE^1_i$ is defined in Equation~\eqref{e:EE}), then $i\in \R_u$. 
Hence $i\in \Rt^1_u\setminus \R_u$ implies $\EE^1_i$ and since $\EE^1_i\subseteq \EEb_{i,\U_i}$ we have
\begin{equation}\label{eq:IU-Rubound}
|\R_u|\geq |\Rt^1_{u}| - \sum_{i\in\Mcc_0}\ident[\EE^1_i]\geq |\Rt^1_u| - \sum_{i\in\Mcc_0}\ident[\EEb_{i,\U_i}]\,.
\end{equation}
%
It follows that
\begin{align}
\Pr\big[\,|\R_u|\leq T\,\big]
&  \leq 
\Pr\bigg[\,|\Rt^1_{u}| - \sum_{i\in\Mcc_0}\ident[\EEb_{i,\U_i}]\leq T\,\bigg]
\leq 
\Pr\big[\,|\Rt^1_{u}|< \tfrac{3 T}{2} \,\big]
+
\Pr\bigg[\,\sum_{i\in\Mcc_0}\ident[\EEb_{i,\U_i}]\geq  \tfrac{T}{2} \,\bigg]
\label{eq:IU-Rubound3}\,.
\end{align}
To bound the second term we use Claim \ref{cl:Ftilde} above, which gives
\begin{equation}\label{eq:IU-Ftildebound}
\Ex\bigg[{\sum_{i\in\Mcc_0} \ident[\EEb_{i,\U_i}]}\bigg]\leq \,\,2\,|\Mcc_0|\, \epsilon = \frac{64T}{N\ell}\,,
\end{equation}
and by Markov's Inequality\footnote{Note that application of Markov's Inequality does not require the events $\EEb_{i,\U_i}$ to be jointly independent for various values of $i\in\Mcc_0$. This is discussed in Remark~\ref{r:usersToItems}. \MK{add one more sentence about the remark!}}
\begin{equation}\label{eq:IU-Ftildebound2}
\Pr\Big[\,\sum_{i\in\Mcc_0} \ident[\EEb_{i,\U_i}]\geq \tfrac T2\,\Big] \leq \frac{128}{ \ell\, N}\,.
\end{equation}
%
%
We now bound the first term on the right-hand side of~\eqref{eq:IU-Rubound3}.
To this end, let 
%$\Rt^1(\ti)$ be the set of items in $\Mcc_0$ whose types are the same as $\rep_{\ti}$:
%\begin{equation} \label{eq:IU-Rj}
%\Rt^1(\ti) =\{i\in\Mcc_0: \tau_I(i)=\tau_I(\rep_{\ti})\}\,.
%\end{equation}
%The sets $\Rt^1(\ti)$ are disjoint because the representatives necessarily have different types. Let 
\begin{equation}
\label{eq:IU-Luk}
\widetilde\Lc_u^{(\ell)}=\{\tau_I(\rep_{\ti}):\ti\in[\ell], L_{u,\rep_{\ti}}=+1\}
\end{equation}
 be the type of item representatives that are liked by user $u$. 
By definition of $\Rt^1_u$ in~\eqref{eq:IU-Ruk},
% $$\Rt^1_u = \bigcup_{\ti\in\widetilde\Lc_u^{(\ell)}} \Rt^1(\ti)\,,$$
%%
%and hence
\begin{equation*}
|\Rt^1_u| = \sum_{i\in\Mcc_0} \ident[\tau_I(i)\in\widetilde\Lc^{(\ell)}_u].
\end{equation*}
Now, we claim that the set $\widetilde\Lc^{(\ell)}_u$ is independent of all items in $\Mcc_0$ and their types.
To see this, note that $\widetilde\Lc^{(\ell)}_u$ is determined by row $u$ of the type matrix $\Xi$ and
the items in $\Mcct_0$, their types, and randomness in the algorithm, which determines the choice of $\rep_{\ti}$ and $\tau_I(\rep_{\ti})$; these together determine $L_{u,\rep_{\ti}}= \xi_{\tau_U(u),\tau_{I}(\rep_{\ti})}$ and $\tau_I(\rep_{\ti})$.
%
%
So, conditioning on $\widetilde\Lc^{(\ell)}_u$ having cardinality $\tilde\ell_u$, $|\Rt_u|$ is the sum of $|\Mcc_0| = 64\frac{\qi }\ell T$ i.i.d. Bernoulli variables with parameter $\frac{\tilde\ell_u}{\qi}$ and hence $|\Rt^1_u|\sim\mathrm{Binom}(64\frac{\qi }\ell T,\frac{\tilde\ell_u}{\qi})$. 
Conditioning on $\tilde\ell_u\geq\frac{\ell}{30}$, by a Chernoff bound (Lemma~\ref{l:Chernoff}) and stochastic domination of binomials with increasing number of trials we obtain
%
\[\Pr\left[|\Rt^1_u| < \tfrac{3 T}{2} \,\Big|\,\tilde\ell_u\geq \tfrac{\ell}{30}\right]
\leq 
\, \exp{\big(-\tfrac{T}{11}\big)}
%\exp(-T/11)
\,.\]
%
In Lemma \ref{cl:IU-lukbd} below, we will lower bound the probability that $\tilde\ell_u\geq {\ell}/{30}$. 
Combining the last displayed inequality with Lemma \ref{cl:IU-lukbd}, we get
\[\Pr\big[|\Rt^1_u| < 3 T/2\big] 
\leq 
\exp{\big(-\tfrac{T}{11}\big)} + 
\exp{\big(-\tfrac{\ell}{5}\big)} 
%\exp(-{\ell}/{5}) 
+ \exp{\big(-\tfrac{\qi}{18}\big)}
%\exp(-{\qi}/{18}) 
+ \frac{20}{N}\,.
\]
Plugging this and~\eqref{eq:IU-Ftildebound2} into~\eqref{eq:IU-Rubound3} gives 
\[\Pr\big[\, |\R_u| < T\big]
\leq 
\exp{\big(-\tfrac{T}{11}\big)} + 
\exp{\big(-\tfrac{\ell}{5}\big)} 
+ \exp{\big(-\tfrac{\qi}{18}\big)}
%\exp(-{T}/{11}) + 
 %\exp(-{\ell}/{5}) + 
 %\exp(-{\qi}/{18}) + 
+ \frac{20}{N} +
\frac{128}{\ell\,N} 
% {128}/{\ell N} 
 \,,\]
and since $\ell$ is less than both $T$ and $\qi\,$ and $\ell>6$
\[\Pr[|\R_u| < T]\leq 3\exp(-{\ell}/{18})+ {148}/{ N} \,.\]
The bound on $\Exp{(T- |\R_u |)_+} $ follows.
\end{proof}
%
\begin{lemma}\label{cl:IU-lukbd}
Fix $u\in[N]$ and suppose that $\qi>8\thr$. 
With $\widetilde\Lc^{(\ell)}_u$ defined in~\eqref{eq:IU-Luk} 
 and $\tilde\ell_u=\big|\widetilde\Lc^{(\ell)}_u\big|$,
\begin{equation*}
\Pr\big[\,\tilde\ell_u< {\ell}/{30}\,\big] \leq \exp(-{\ell}/{5}) + \exp(-{\qi}/{18})+ {20}/{N}\,.
\end{equation*}
\end{lemma}
%
\begin{proof}
For a given user $u$, $\tilde\ell_u$ is the number of item type representatives liked by user $u$. 
%
Let $\Lc_u$ be the item types in $[\qi]$ that are liked by user $u$: 
\begin{equation}
\Lc_u= \{\ti\in[\qi]: \xi_{\tau_U(u),\ti}=+1 \}\,.
\end{equation}
%
The variables $\{\xi_{\tau_U(u),j}\}_{j\in [\qi]}$ are i.i.d.  $\mathrm{Bern}(1/2)$, so a Chernoff bound (Lemma \ref{l:Chernoff}) gives 
\begin{equation}
\label{eq:IU-Lcubd}
\Pr\big[\,|\Lc_u|< {\qi}/{3}\,\big]
<
 \exp(-{\qi}/{18})\,.
\end{equation}
%
We will show that 
\begin{equation}\label{eq:IU-ell-condLu}
\Pr\big[\tilde\ell_u \leq {\ell}/{30} \,\big|\, |\Lc_u|
\geq {\qi}/{3}\big] \leq \exp(-{\ell}/{5}) + {20}/{N}\,,
\end{equation}
which will prove the lemma by combining with \eqref{eq:IU-Lcubd}.
%

We now work towards defining a certain error event in Equation~\eqref{def:IU-iuerr} below.
Let the sequence of random variables $X_1 = \tau_I(\rep_1), X_2 = \tau_I(\rep_2), \dots, X_{\ell}=\tau_I(\rep_{\ell})$ denote the types of the item representatives chosen by the algorithm, so that 
$\tilde\ell_u=|\widetilde\Lc^{(\ell)}_u| = \sum_{\ti\in[\ell]}\ident[X_{\ti}\in \Lc_u]$
 (with $\widetilde\Lc^{(\ell)}_u$ defined in~\eqref{eq:IU-Luk}). 
%
Let $\Rb^2(\ti)$ be the set of items in $\Mcct_0$ of type $\ti$
\begin{equation}\label{IU-Rb2}
\Rb^2(\ti)= \{i\in\Mcct_0:\tau_I(i)=\ti\}\,.
\end{equation}
Later we will use the notation 
$\Rb^2(\cdot)= \{\Rb^2(j)\}_{j=1}^{\qi}$ 
for the collection of these sets.
Now let the event $\EE^2_i$ denote misclassification of an item $i\in\Mcct_0$ (similar to event $\EE^1_i$ for $i\in\Mcc_0$ in~\eqref{e:EE}),
	\begin{equation}\label{e:EEt}
		\EE^2_i = \{\exists \ti : i\in{\mathcal{S}}^2_\ti, \tau_I(i)\neq \tau_I(\rep_\ti)\}\,.
		\end{equation}
%		
Let $\iuerr$ be the event that for some item type $\ti$, more than a fraction $1/10$ of the items in $\Mcct_0$ of type $\ti$ are misclassified:
\begin{equation}\label{def:IU-iuerr}
\iuerr = \bigg\{\sum_{i\in\Rb^2(\ti)}\ident[\EE^2_i]> \frac{|\Rb^2(\ti)|}{10}, \text{ for some } \ti\in[\qi]\bigg\}.
\end{equation}
%
%
%
Conditioning on $\iuerr$ in the left-hand side of \eqref{eq:IU-ell-condLu} gives
\begin{align}
 &\Pr\bigg[\sum_{i=1}^{\ell}\ident\big[X_i\in\widetilde\Lc^{(\ell)}_u\big]<\ell/30 \, \bigg|\,  |\Lc_u|\geq \qi/3\bigg] \notag
 \\
& \leq \Pr\bigg[\,\,\sum_{i=1}^{\ell}\ident\big[X_i\in\widetilde\Lc^{(\ell)}_u\big]<\ell/30 \, \bigg|\, \iuerr^c , |\Lc_u|\geq \qi/3\bigg] 
+
 \Pr\Big[\,\iuerr \,\,\Big|\, |\Lc_u|\geq \qi/3\,\Big]\,.
\label{e:errTemp}
\end{align}


\paragraph{Bound on second term of \eqref{e:errTemp}.}
We will use Markov's inequality to bound 
$$\Pr\Big[\,\iuerr \,\Big|\, |\Lc_u|\geq \qi/3\,\Big] = \Exp{\Pr\big[\,\iuerr\,\big|\,\tau_I(i),\Rb^2(\cdot), {\Lc}_u \,\big] \,\Big|\, |\Lc_u|\geq \qi/3 }\,.$$
We need to consider the effect of matrix $\Xi$ (and in particular its $\tau_U(u)$th row, which determines $\Lc_u$) on the probability of error in categorizing items. 
Notably, if users rate two item types similarly, the probability of misclassifying these types is higher. 
As a result, ${\Lc}_u$ contains some information about discriminability of distinct item types and we need to control this dependence.

Claim \ref{cl:iu-error-indep2} shows that for $i\in\Mcc_0$, the probability of $\EE^1_i$ (the event that item $i$ is miscategorized) is $\Pr[\EE^1_i]\leq 2\epsilon$. 
The same proof gives $\Pr[\EE^2_i]\leq 2\epsilon$ (with $\EE^2_i$ defined in~\eqref{e:EEt} for $i\in\Mcct_0$). 
To show that,
   let the potential error event $\EEb_{i,U_i}$, be the event that there exists an item type $\ti\neq \tau_I(i)$ such that for all the users $u$ in $U_i$, we have $L_{u,i}=\xi_{\tau_U(u),\ti}$. 
      For $i\in{\S}^2_{\ti}$, let $U_i=\rated(i)\cap\rated(\rep_{\ti})$ at the time the algorithm added $i$ to ${\S}^2_{\ti}$. 
Then the containment $\EE^2_i\subseteq\EEb_{i,U_i}$ holds. 
We will later use the inequality $\Pr[\EE^2_i | \tau_I(i), \Rb^2(\cdot),{\Lc}_u]\leq \Pr[\EEb_{i,\U_i} | \tau_I(i), \Rb^2(\cdot),{\Lc}_u]$ and focus on the set of users 
$\U_i\setminus\{u\}$, using 
$\EEb_{i,\U_i}\subseteq \EEb_{i,\U_i\setminus \{u\}}$. 
%=\Pr[\EEb_{i,U_i} | {\Lc}_u]$, where the equality follows because the event $\EEb_{i,U_i}$ is independent of $\Rb^2(\cdot)$ ($\EEb_{i,U_i}$ is a function of $\Xi,U_i$, $\tau_U(u)$ for $u\in U_i$ and $\tau_I(i)$ for $i\in \Mcct_0$, while $\Rb(\cdot)$ is a function of $\tau_I(i)$ for $i\in\Mcc1$). 
%
%
%We will later use the inequality $\Pr[\EE^2_i | \Rb^2(\cdot),{\Lc}_u]\leq \Pr[\EEb_{i,U_i} | \Rb^2(\cdot),{\Lc}_u]=\Pr[\EEb_{i,U_i} | {\Lc}_u]$, where the equality follows because the event $\EEb_{i,U_i}$ is independent of $\Rb^2(\cdot)$ ($\EEb_{i,U_i}$ is a function of $\Xi,U_i$, $\tau_U(u)$ for $u\in U_i$ and $\tau_I(i)$ for $i\in \Mcct_0$, while $\Rb(\cdot)$ is a function of $\tau_I(i)$ for $i\in\Mcc1$). 

As specified in Algorithm $\textsc{ItemExplore}$, 
for each $i\in \Mcc_0\cup \Mcct_0$ the set $\U_i$ of at least $\thr$ users, chosen independently of feedback, rate item $i$. 
By Lemma~\ref{l:ballsbins}, if $\qu>4\thr$, then
there are users of at least $\thr/2$  distinct user types in $\U_i$ with probability at least $1-\exp(-\thr/2)\geq 1-\epsilon/\qi\,.$
%
%To bound  $\Pr[ \EEb_{i,U_i\setminus \{u\}} | \tau_I(i), \Rb^2(\cdot),{\Lc}_u]$, we 
Conditional on $\U_i$ having at least $\thr/2$  distinct user types, there are at least $\thr/2-1$ users of distinct types in $\U_i\setminus\{u\}$---also distinct from type of $u$---whose preferences for item type $\tau_I(i)$ are independent of ${\Lc}_u$ and $\Rb^2(\cdot)$.

Conditional on $ \tau_I(i), \Rb^2(\cdot),{\Lc}_u$, any two item types $\ti\neq \ti'$ have jointly independent user preferences by $\thr/2-1$ users with distinct types  in $\U_i\setminus\{u\}$; 
they are rated in the same way by these users with probability at most $2^{-(\thr/2-1)}$. 
A union bound over item types $\ti'\neq\tau_I(i)$  gives $\Pr[ \EEb_{i,\U_i\setminus \{u\}} | \tau_I(i), \Rb^2(\cdot),{\Lc}_u]\leq \qi 2^{-(\thr/2-1)}$.
The choice $\thr>2\log(\qi/\epsilon)$ and $\epsilon=\frac{1}{2\qi N}$ and the containment 
$\EE^2_i \subseteq \EEb_{i,\U_i} \subseteq \EEb_{i,\U_i\setminus \{u\}}$
gives 
$\Pr[\EE^2_i | \tau_I(i), \Rb^2(\cdot),{\Lc}_u]\leq \frac{1}{\qi N}$ for all $i\in\Mcct_0$.
Markov's inequality gives
\[\Pr\bigg[\,\sum_{i\in\Rb^2(\ti)} \ident[\EE^2_i] >\frac{|\Rb^2(\ti)|}{10} \, \bigg| \,\tau_I(i), \Rb^2(\cdot), {\Lc}_u\,\bigg] \leq \frac{20}{\qi N}\,.\]
Union bounding over $\ti\in[\qi]$ and tower property gives the desired bound.

%To bound  $\Pr[\EEb_{i,U_i} |\widetilde{\Lc}_u]$, we focus on the set of users $U_i\setminus\{u\}$. Conditional on $U_i$ having at least $\thr/2$  distinct user types, there are at least $\thr/2-1$ users of distinct types in $U_i\setminus\{u\}$---also distinct from type of $u$---whose preferences for item $i$ are independent of $\widetilde{\Lc}_u$. Any two item types $\ti\neq \ti'$ have jointly independent user preferences by $\thr/2-1$ users with distinct types  in $U_i\setminus\{u\}$; they are rated in the same way by these users with probability at most $2^{-(\thr/2-1)}$. Hence, a union bound over item types $\ti'\neq\tau_I(i)$  gives $\Pr[\EEb_{i,U_i} | \widetilde{\Lc}_u]\leq \qi 2^{-(\thr/2-1)}$.
%The choice $\thr>2\log(\qi/\epsilon)$ and $\epsilon=\frac{1}{2\qi N}$ gives $\Pr[\EEb_{i,U_i} | \widetilde{\Lc}_u]\leq \frac{1}{\qi N}$. So, $\Pr[\EEt_i | \Rb(\cdot),\widetilde{\Lc}_u]\leq \frac{1}{\qi N}$ for all $i\in\Mcc{1}$.
%Markov's inequality gives
%\[\Pr\bigg[\,\sum_{i\in\Rb(\ti)} \ident[\EEt_i] >\frac{|\Rb(\ti)|}{10} \, \bigg| \,\Rb(\cdot), \widetilde{\Lc}_u\,\bigg] \leq \frac{20}{\qi N}\,.\]
%Union bounding over $\ti\in[\qi]$ and tower property gives the desired bound.

\paragraph{Bound on first term of \eqref{e:errTemp}.}
We start by showing that conditioned on the event $\iuerr^c$ conditional on  $\Lc_u$ and variables $X_1,\cdots,X_{m-1} $ and $ \Rb^2(X_1),\cdots, \Rb^2(X_{m-1})$, the type of the $m$-th representative item, $X_m$, is almost uniform over all the item types not learned yet, $\ti\in [\qi]\setminus\{X_1,\cdots,X_{m-1}\}$. 
%We start by showing that conditioned on the event $\iuerr^c$, variables $\Rb(\cdot)$, $\widetilde\Lc_u$ such that $|\widetilde\Lc_u|\geq \qi/3 $ and conditional on $X_1,\cdots,X_{m-1}$, the type of the $m$th representative item, $X_m$, is almost uniform over all the item types not learned yet, $[\qi]\setminus\{X_n\}_{n=1}^{m-1}$. 
%
Concretely, we will find upper and lower bounds on
\begin{equation}\label{eq:IU-nextrep}
\Pr\big[X_{m}=\ti \,\,\big|\, \big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, \,\Lc_u\,, \iuerr^c\,\big]
\end{equation}
for any $\ti\in [\qi]\setminus\{X_1,\cdots,X_{m-1}\}$. Later, we will focus on $\Lc_u$ such that $|\Lc_u|\geq \qi/3$.

%
\emph{Lower bound for~\eqref{eq:IU-nextrep}.}
Let $t$ be the time the $m$-th item type representative is chosen by the algorithm. For $\ti\in [\qi]\setminus\{X_n\}_{n=1}^{m-1}$ the probability of choosing representative of type $X_m=\ti$ is equal to the proportion of items of type $\ti$ in the remaining items in $\Mcct$ at time $t-1\,.$ 
The number of items of type $\ti$ in $\Mcct$ at time $t-1$ is at least $|\Rb^2(\ti)|- \sum_{i\in\Rb^2(\ti)}{\ident[\EE^2_i]}$. 

The number of items removed from $\Mcct$ by time $t$ is at least $\sum_{l=1}^{m-1}|\Rb(X_l)|$ (there could be additional items with types not in $\{X_n\}_{n=1}^{m-1}$ that were removed from $\Mcct$ due to misclassification). Hence, the total number of remaining items in $\Mcct$ by time $t$ is at most $M - \sum_{n=1}^{m-1}|\Rb^2(X_n)|$. Let $Z_{\EE^2}$ be the collection of indicator variables $Z_{\EE^2} = \{\ident_{\EE^2_i}\}_{i\in\Mcct_0}$. 
For any $\ti\in [\qi]\setminus\{X_n\}_{n=1}^{m-1}$:
\begin{align*}
\Pr\Big[X_m=\ti  \,\big|\,
\big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, 
\Lc_u,  Z_{\EE^2}\Big]
 \geq \frac{|\Rb^2(\ti)|- \sum_{i\in\Rb^2(\ti)}{\ident[\EE^2_i]}}{M - \sum_{n=1}^{m-1}|\Rb^2(X_n)|} \,.
\end{align*}
On the event $\iuerr^c$ (defined in~\eqref{def:IU-iuerr}), 
$\sum_{i\in\Rb^2(\ti)}{\ident[\EE^2_i]}\leq |\Rb^2(\ti)|/10$ 
for any $\ti\in [\qi]\setminus\{X_n\}_{n=1}^{m-1}$. 
Therefore, \begin{align}\label{eq:IU-luKj1}
\Pr\Big[X_m=\ti\,\big|\,
\big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, 
\Lc_u, \iuerr^c\Big]
\geq \frac{|\Rb^2(\ti)|}{M - \sum_{n=1}^{m-1}|\Rb^2(X_n)|}\frac{9}{10}\,.
\end{align}

\noindent\emph{Upper bound for~\eqref{eq:IU-nextrep}.} 
This time we lower bound the number of items remaining in $\Mcct$ by the number of items in types $[\qi]\setminus\{X_n\}_{n=1}^{m-1}$ minus the number of possible mistakes which removed some items from them. This gives
\begin{align*}
\Pr\Big[X_m=\ti  
\,\big|\,
\big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, 
\Lc_u,  Z_{\EE^2} \Big]
 \leq 
 \frac{|\Rb^2(\ti)|    \substack{j\\jh}}
 {M - 
 \sum\limits_{n=1}^{m-1}|\Rb^2(X_n)| - 
 \sum\limits_{\substack{i\in\Mcct_0\setminus  \cup_{n=1}^{m-1}\Rb^2(X_n)}}{\ident[\EE^2_i]}} \,.
\end{align*}
By definition of $\iuerr$ (in~\eqref{def:IU-iuerr}), we have
\begin{align}\label{eq:IU-luKj2}
\Pr\Big[X_m=\ti\,\big|\,&
\big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, 
 \Lc_u, \iuerr^c\Big]
\leq  \frac{10}{9}\frac{|\Rb^2(\ti)|}{M - \sum_{n=1}^{m-1}|\Rb^2(X_n)|}\,.
\end{align}

\noindent \emph{Combining lower and upper bounds.}
The expected value of $|\Rb^2(\ti)|$ conditional on variables $\{X_n\}_{n=1}^{m-1}$, $\{\Rb^2(X_n)\}_{n=1}^{m-1}$, and $\Lc_u$ is invariant to choice of $\ti\in [\qi]\setminus\{X_n\}_{n=1}^{m-1}$. So, the conditional expectation
$$C = 
\Exp{\frac{|\Rb^2(\ti)|}
{M - \sum_{n=1}^{m-1}|\Rb^2(X_n)|}  \bigg|
\big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, 
\Lc_u,\iuerr^c},$$
 is independent of $\ti$ for $\ti\in [\qi]\setminus\{X_n\}_{n=1}^{m-1}$. 
Using tower property of expectation on~\eqref{eq:IU-luKj1} and~\eqref{eq:IU-luKj2} to remove the conditioning on 
$\{\Rb(j)\}_{j\notin \{X_n\}_{n=1}^{m-1}}$ 
along with the definition of $C$ above gives
\[\frac{9}{10}C
\leq 
\Pr\Big[X_m=\ti\, \Big|\,
\big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, 
\Lc_u,\iuerr^c\Big] 
\leq
\frac{10}{9}C \,.\]
Since there are $\qi - (m-1)$ types $\ti\in [\qi]\setminus\{X_n\}_{n=1}^{m-1}$, summing over $\ti$ in the second inequality of the last display gives  $C\geq\frac{9}{10}\frac{1}{\qi-(m-1)}$. Plugging this into the first inequality of the last display gives for all $\ti\in [\qi]\setminus\{X_n\}_{n=1}^{m-1}$,
%
%
	\begin{align*}
\Pr\Big[X_m=\ti\, \Big|\,
\big\{X_n\big\}_{n=1}^{m-1}, \big\{\Rb^2(X_n)\big\}_{n=1}^{m-1}, 
\Lc_u,\iuerr^c\Big] 
&>\frac{2}{5}
\frac{1}{\qi- m+1}\,.
\end{align*}
Conditional on $\Lc_u$ such that $|\Lc_u|\geq \qi/3,$ for $m\leq\ell\leq \qi$ and $s\leq\ell/30$ we have
\begin{align*}
\Pr\bigg[X_m\in\Lc_u 
\,\bigg|\,
\{X_n\}_{n=1}^{m-1}, \sum_{n=1}^{m-1}\ident[X_{n}\in\Lc_u] < s, \Lc_u, |\Lc_u|\geq \qi/3, \iuerr^c\bigg] 
\geq \frac{2}{5}\frac{\frac{\qi}{3}-\min\{m,\ell/30\}}{\qi-m+1}\geq \frac{1}{9}\,.
\end{align*}
So, on the event $\sum_{n=1}^{\ell}\ident[X_{n}\in\Lc_u] \leq\frac{\ell}{30} $, 
the random variable $\sum_{n=1}^{\ell}\ident[X_{n}\in\Lc_u]$  conditional on $\Lc_u$ and events $ |\Lc_u|\geq \qi/3$ and $ \iuerr^c$,  stochastically dominates a Binomial random variable with mean $\ell/9$. Hence, by a Chernoff bound,
\[
\Pr\bigg[\sum_{n=1}^{\ell}\ident[X_{n}\in\Lc_u] \leq \frac{\ell}{30} 
\,\bigg|\, 
\Lc_u, |\Lc_u|\geq \frac{\qi}{3}, \iuerr^c\,\bigg] 
\leq  
\exp(-\ell/5)\,.\qedhere\] 
\end{proof}
%
